Chordal Decomposition for Spectral Coarsening

We introduce a novel solver to significantly reduce the size of a geometric operator while preserving its spectral properties at the lowest frequencies. We use chordal decomposition to formulate a convex optimization problem which allows the user to control the operator sparsity pattern. This allows for a trade-off between the spectral accuracy of the operator and the cost of its application. We efficiently minimize the energy with a change of variables and achieve state-of-the-art results on spectral coarsening. Our solver further enables novel applications including volume-to-surface approximation and detaching the operator from the mesh, i.e., one can produce a mesh tailormade for visualization and optimize an operator separately for computation.

==> EG_latex/derekPre.tex <==
\usepackage{wrapfig}
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{graphicx}
\usepackage{booktabs} 
\usepackage{combelow} % for comma underneath a word
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{tabularx} % beautiful table
\usepackage{colortbl} % add row color to a table

\usepackage{manfnt} % cube symbol

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}


% for unicode math symbols
% \usepackage[mathletters]{ucs}
% \usepackage[utf8x]{inputenc}

\definecolor{derekBlue}{RGB}{144,210,236}
\definecolor{honglinPurple}{RGB}{115, 113, 235}
\definecolor{derekTableBlue}{RGB}{189,235,252}
\definecolor{iglGreen}{RGB}{153,203,67}
\definecolor{coralRed}{RGB}{250,114,104}
\definecolor{gray}{RGB}{180,180,180}
\definecolor{alecGreenn}{RGB}{51,204,51}


% set algorithm2e comment style
% \newcommand\commentFont[1]{\itshape\textcolor{gray}{#1}}
% \SetCommentSty{commentFont}
% \SetNlSty{textbf}{}{.}

\newcommand{\derek}[1]{{\color{derekBlue}Derek: #1}}
\newcommand{\note}[1]{{\color{derekBlue}#1}}
\newcommand{\gray}[1]{\text{\color{gray}#1}}
\newcommand{\alec}[1]{{\color{alecGreenn}Alec: #1}}
\newcommand{\honglin}[1]{{\color{honglinPurple}Honglin: #1}}
% \newcommand{\alec}[1]{{\textcolor[rgb]{0.2,0.8,0.2}{Alec: #1}}}

\newcommand{\refequ}[1] {Eq.~\ref{equ:#1}}
\newcommand{\refequnum}[1] {\ref{equ:#1}}
\newcommand{\reffig}[1] {Fig.~\ref{fig:#1}}
\newcommand{\reffignum}[1] {\ref{fig:#1}}
\newcommand{\reftab}[1] {Table~\ref{tab:#1}}
\newcommand{\refsec}[1] {Sec.~\ref{sec:#1}}
\newcommand{\refapp}[1] {App.~\ref{app:#1}}
\newcommand{\refalg}[1] {Alg.~\ref{alg:#1}}
\newcommand{\refthm}[1] {Theorem~\ref{thm:#1}}

% my math symbols
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\newtheorem{theorem}{Theorem}

% reserved symbols
\newcommand{\R}{\mathbb{R}} % real number
\newcommand{\C}{\mathcal{C}} % chordal sparsity
\newcommand{\E}{\mathcal{E}} % original sparsity
\newcommand{\N}{\mathcal{N}} % dense sparsity

\newcommand{\X}{\mX} % original system matrix
\newcommand{\x}{\vx} % vec(X) 
\newcommand{\xE}{\vx_{\E}} % reduced vec(X) to only the sparsity pattern E
\newcommand{\sx}{x} % set x

\newcommand{\Z}{\mZ} % Z matrix
\newcommand{\rZ}{\widetilde{\mZ}} % Z vector
\newcommand{\z}{\vz} % Z vector
\newcommand{\rz}{\tilde{\vz}} % Z vector
\newcommand{\y}{\vy} % Z vector
\newcommand{\ry}{\tilde{\vy}} % Z vector
\newcommand{\ru}{\tilde{\vu}} % Z vector

\renewcommand{\S}{\mathbb{S}} % symmetric

\renewcommand{\i}{i} % ith clique set

\renewcommand{\P}{\mP} % selection matrix
\newcommand{\invP}{\mP^{\text{-}1}} % \text{vec}(\X) = \invP_{\sX} \xE
\newcommand{\Q}{\mQ} % selection matrix
\newcommand{\invQ}{\mQ^{\text{-}1}} % \text{vec}(\X) = \invP_{\sX} \xE
\newcommand{\K}{\mK} % P otimes P
\newcommand{\rK}{\widetilde{\mK}} % P otimes P
\newcommand{\s}{s} % set

\newcommand{\PhiE}{\tilde{\Phi}} % coarsened system matrix

% Old symbols
\newcommand{\cl}{Z} % cliques
\newcommand{\clvec}{z} % cliques for vectors
% \newcommand{\K}{k} % Z matrix
\renewcommand{\k}{k} % Z vector
\newcommand{\Pm}{\mP} % selection matrix for matrices
\newcommand{\Pv}{\widetilde{\mP}} % selection matrix for vectors
\newcommand{\q}{q} % clique set
\newcommand{\sZ}{K} % set Z
\newcommand{\sz}{k} % set z
\newcommand{\sX}{X} % set X
\newcommand{\sxE}{\tilde{x}} % set xE
\newcommand{\XE}{\tilde{\X}} % coarsened system matrix

% vectors
\newcommand{\vecFont}[1]{\mathbf{#1}}
\def\va{{\vecFont{a}}}
\def\vb{{\vecFont{b}}}
\def\vc{{\vecFont{c}}}
\def\vd{{\vecFont{d}}}
\def\ve{{\vecFont{e}}}
\def\vf{{\vecFont{f}}}
\def\vg{{\vecFont{g}}}
\def\vh{{\vecFont{h}}}
\def\vi{{\vecFont{i}}}
\def\vj{{\vecFont{j}}}
\def\vk{{\vecFont{k}}}
\def\vl{{\vecFont{l}}}
\def\vm{{\vecFont{m}}}
\def\vn{\hat{\vecFont{n}}}
\def\vo{{\vecFont{o}}}
\def\vp{{\vecFont{p}}}
\def\vq{{\vecFont{q}}}
\def\vr{{\vecFont{r}}}
\def\vs{{\vecFont{s}}}
\def\vt{{\vecFont{t}}}
\def\vu{{\vecFont{u}}}
\def\vv{{\vecFont{v}}}
\def\vw{{\vecFont{w}}}
\def\vx{{\vecFont{x}}}
\def\vy{{\vecFont{y}}}
\def\vz{{\vecFont{z}}}

% matrices
% Matrix
\newcommand{\matFont}[1]{\mathbf{#1}}
\def\mA{{\matFont{A}}}
\def\mB{{\matFont{B}}}
\def\mC{{\matFont{C}}}
\def\mD{{\matFont{D}}}
\def\mE{{\matFont{E}}}
\def\mF{{\matFont{F}}}
\def\mG{{\matFont{G}}}
\def\mH{{\matFont{H}}}
\def\mI{{\matFont{I}}}
\def\mJ{{\matFont{J}}}
\def\mK{{\matFont{K}}}
\def\mL{{\matFont{L}}}
\def\mM{{\matFont{M}}}
\def\mN{{\matFont{N}}}
\def\mO{{\matFont{O}}}
\def\mP{{\matFont{P}}}
\def\mQ{{\matFont{Q}}}
\def\mR{{\matFont{R}}}
\def\mS{{\matFont{S}}}
\def\mT{{\matFont{T}}}
\def\mU{{\matFont{U}}}
\def\mV{{\matFont{V}}}
\def\mW{{\matFont{W}}}
\def\mX{{\matFont{X}}}
\def\mY{{\matFont{Y}}}
\def\mZ{{\matFont{Z}}}

